Bandit Linear Optimization for Sequential Decision Making and Extensive-Form Games

Tree-form sequential decision making (TFSDM) extends classical one-shot decision making by modeling tree-form interactions between an agent and a potentially adversarial environment. It captures the online decision-making problems that each player faces in an extensive-form game, as well as Markov decision processes and partially-observable Markov decision processes where the agent conditions on observed history. Over the past decade, there has been considerable effort into designing online optimization methods for TFSDM. Virtually all of that work has been in the full-feedback setting, where the agent has access to counterfactuals, that is, information on what would have happened had the agent chosen a different action at any decision node. Little is known about the bandit setting, where that assumption is reversed (no counterfactual information is available), despite this latter setting being well understood for almost 20 years in one-shot decision making. In this paper, we give the first algorithm for the bandit linear optimization problem for TFSDM that offers both (i) linear-time iterations (in the size of the decision tree) and (ii) $O(\sqrt{T})$ cumulative regret in expectation compared to any fixed strategy, at all times $T$. This is made possible by new results that we derive, which may have independent uses as well: 1) geometry of the dilated entropy regularizer, 2) autocorrelation matrix of the natural sampling scheme for sequence-form strategies, 3) construction of an unbiased estimator for linear losses for sequence-form strategies, and 4) a refined regret analysis for mirror descent when using the dilated entropy regularizer.

==> text/neurips_cover_letter.tex <==

\section*{Response Document}

Since the previous NeurIPS submission, we made the following main changes to the manuscript:

\begin{itemize}
    \item We added a more detailed comparison of the MCCFR algorithm to our bandit convex optimization method. We added emphasizes to the difference of the \emph{online} MCCFR algorithm used in our experimental evaluation and other MCCFR variants.
    \item 
    \item
\end{itemize}


\subsection*{Response to NeurIPS20 reviewers}
In the following, we provide answers to the questions and concerns of the NeurIPS Reviewers.\\

% Reviewer 1
% ------------------------------------------------------------------------------------
\noindent \textbf{[R1] Clarification: Comparison to ``Theorem 28.10'' Lattimore and Szepesvári's excellent Bandit Algorithms}\\

\noindent Lattimore and Szepesvári's excellent book proposes a \emph{framework} for constructing bandit algorithms similar to (and perhaps inspired by) the framework by Abernethy et al. that we used. Before the mentioned theorem is applicable, several pieces have to be filled in. Our paper gives solutions for some of those missing pieces for our setting---so that theorem was not applicable to our setting before. As one example, Theorem 28.10 requires that an unbiased estimator for the loss vector be available. One of the main contributions of our paper is exactly a construction for that critical piece (Section 4 and Appendix E). Constructing an unbiased estimator with bounded (local) norm and that would play well with OMD was itself a major effort, that took more than four months.\\

\noindent \textbf{[R1] Critique: ``\dots considering only the loss l.x the sequential decisions have effectively been collapsed''}\\

\noindent The reviewer's claim is not correct. The presence of observation points in SDM fundamentally changes the properties of the set of decisions and makes bandit optimization significantly harder. For example, because of the observation points, the number of strategies that can be used by the agent grows exponentially in the size of the decision tree, and sequential decisions cannot be ``\emph{collapsed}''. Balancing the combinatorial intuition behind strategies with the continuous, analytical, details of the set they span, is challenging.\\

\noindent SDM is a natural and widely used model that captures, among others, extensive-form games. Unlike the usual one-shot decision making domain (multi-armed bandit), where one agent faces only one decision point in each repetition of the decision process, in SDM at each iteration the agent interacts with the environment several times (both by picking actions and by observing signals) before getting feedback. Hence, at each repetition, it is not enough for the agent to output the selected arm for the multi-armed bandit, and instead the agent has to formulate a full decision tree, contingent on what the agent might observe from the environment.\\

\noindent \textbf{[R1] Request: Experimental comparison with EXP3 algorithm.}\\

\noindent As noted on Section 4, our algorithm coincides with EXP3 when the decision process only has one decision point.\\

\noindent \textbf{[R1, R3, MR1] Clarification: MCCFR seems to define a complete strategy at every iteration.}\\

\noindent MCCFR can also be used for \emph{interactive} game playing, which is a nice feature that our algorithm does not possess. On the other hand, our algorithm operates in a more difficult setting (bandit linear optimization), so there is a trade-off. We find that being able to achieve $O(\sqrt{T})$ regret in \emph{sequential} decision making with so little feedback is mind bending.\\

\noindent \textbf{[R1, R2, R3] Clarification: How does exploration in MCCFR effect the regret.}\\

\noindent Adding $\epsilon$-exploration in MCCFR has two effects: (i) the norm of the unbiased loss estimates (and therefore, regret updates) degrades roughly as $1/\epsilon^d$ (where $d$ is the maximum depth of the game); (ii) there is an additive error term of the order of $\epsilon T$ due to the fact that the agent is not following the strategy output by CFR but is instead introducing some biasing. Hence, there is no way of setting $\epsilon$ so as to guarantee that $\sqrt{T}/\epsilon^d + \epsilon T \in O(\sqrt{T})$, which our algorithm guarantees. To sidestep this issue, we avoided using exploration altogether. MCCFR seems to perform well even without exploration, as we showed in the paper. See also next answer.\\

\noindent \textbf{[R1, R2, R3] Request: How was exploration for MCCFR handled in the experiments?}\\

\noindent We didn't use exploration in MCCFR. MCCFR was included as a baseline, but it is somewhat outside of the scope of the paper since it is \emph{not} an algorithm for bandit linear optimization. It requires more feedback,  but leads to faster performance in practice, as we show. Also, as far as we're aware, we are the first to implement AHR (at least in SDM domains), and compare bandit algorithms to MCCFR. Of course, we think this is a minor contribution compared to all the theoretical groundwork in the paper.\\

\noindent \textbf{[R1] Request: How many iterations did each algorithm use?}\\

\noindent For the non-anytime algorithms (ours and AHR), we divided the desired runtime (e.g., 3 hours in Leduc poker) by the average time per iteration of each algorithm. We'll include this detail in the final version.\\

\noindent \textbf{[R1] Request: How where parameters selected for the individual methods?}\\

\noindent Parameters were tuned for all the algorithms to be fair. However, the tuning did not make much difference. It is important to note that the tuned parameters are still theoretically sound.\\

\noindent \textbf{[R1] Request: Which units are displayed on the y-Axis of Figure 1?}\\

\noindent It is regret in natural units / $T$. We'll include this detail.\\


% Reviewer 2
% ------------------------------------------------------------------------------------

\noindent \textbf{[R2] Clarification: Comparison to AHR algorithm.}\\

\noindent AHR is the algorithm that was proposed by Abernethy et al. in 2008. We propose a different algorithm. Our algorithm has stronger theoretical guarantees than AHR, is numerically stable, and guarantees lower run time per iteration both in theory and practice. However, our algorithm is specific to SDM. Also, in the process of developing our algorithm, we extend several existing theoretical tools that have been traditionally used in SDM, such as the dilated entropy regularizer. Also, we achieve $O(\sqrt{T})$ regret, not just $O(T)$ as you write in the summary.\\

\noindent \textbf{[R2] Critique: MCCFR was not used with external sampling and robust sampling.}\\

\noindent Out of those methods, only outcome sampling can be used in an online fashion in a bandit setting like ours (this is also stated by the original MCCFR authors). The other sampling schemes are \emph{off-policy} and cannot be used in the bandit setting we are studying. The problem with off-policy exploration is that in our setting we do not control the opponent: after we output our strategy, the opponent reacts and changes policy---we can't go back and sample another strategy for us to construct an unbiased estimator. The environment can be queried only once per iteration, and the interaction is final. We'll complement our discussion of MCCFR (Lines 110-122) with this discussion, and cite robust sampling. This is also the reason why in the experiments we only consider outcome sampling. Also, MCCFR, regardless of the sampling scheme, is not an algorithm for bandit linear optimization, so the comparison of AHR and our algorithm against MCCFR is not apples-to-apples: we give MCCFR extra feedback in that test.\\

\noindent \textbf{[R2] Critique: The size of the decision tree grows exponentially and this is the main challenge in SDM. No evaluation on larger games.}\\

\noindent The number of strategies that can be employed in an SDM problem is exponential in the SDM size. However, our algorithm runs in polynomial time (in fact, linear time!) in the SDM size. Being able to efficiently design an algorithm that can operate over an exponential number of strategies without enumerating them was one of the challenges.\\
    
\noindent The main obstacle against trying on larger games is that AHR (the only previously known algorithm for our setting that achieves (i) iterations that are polynomial in the number of sequences in the decision process and (ii) $\tilde{O}(\sqrt{T})$ expected regret) becomes prohibitively slow since it runs in cubic time per iteration instead of linear time like our algorithm. So, our algorithm is the only bandit linear optimization algorithm with optimal $O(\sqrt{T})$ (in-expectation) regret guarantees that can scale to large SDM problem. Such experiments would not have any bandit algorithm to compare against.\\

\noindent \textbf{[R2] Clarification: How is choice of weights in the dilated entropy regularizer motivated.}\\

\noindent The choice of weights comes directly from the original work by Kroer et al.. It guarantees that the regularizer is $1$-strongly convex on the set of strategies.\\

\noindent \textbf{[R3] Critique: No comparison with experience sampling based methods.}\\

\noindent What you write is true. However, there is another valuable reason to care about the bandit optimization setting: it is a more restrictive setting. In bandit optimization for SDM, only on-policy exploration is allowed, and the feedback is minimal. So, by conquering the bandit optimization setting (and being able to guarantee $O(\sqrt{T})$ regret in linear time per iteration), in theory we are also conquering all the less restrictive settings.\\

\noindent \textbf{[R3] Request: Additional references on MCCFR for quantal-response equilibria}\\

\noindent Thank you for the pointers, we'll cite them and amend the writing.\\

\noindent \textbf{[R3] Request: Clarify that regret might not converge for any algorithm that does not enjoy a high-probability regret bound.}\\

\noindent Thank you for the feedback, we'll use a more precise wording.\\ 

\noindent \textbf{[R3] Clarification: The Leduc game used in experiments has been reduced to its canonical form, correct?}\\

\noindent Yes, we were referring to the action space of each player.\\

\noindent \textbf{[R4] Critique: No high probability bound was shown.}\\

\noindent We hope that our analytical and combinatorial results about some of the fundamental tools in SDM will pave the way to high-probability results as well. We will investigate this direction in the future.\\


==> text/neurips_reviews.tex <==
\section{NeurIPS2020 Reviews}

% TODO: Mark critique point in the reviews and discuss those in an additional cover letter

% Reviewer 1
% --------------------------------------------------------------------------------------

\subsection{Reviewer \#1}

\noindent \textbf{1. Summary and contributions: Briefly summarize the paper and its contributions.}\\
\noindent This paper gives:
i) a regret bound for OMD over sequence form strategies using dilated entropy as a regulariser.
ii) a more general way to construct a loss estimate in the bandit case for the underlying OMD algorithm, given the observed loss.
iii) a theorem connecting the pieces of a sampled OMD algorithm for sequence form bandit problems, giving a bound on expected regret.
iv) experimental results\\
 
\noindent \textbf{2. Strengths: Describe the strengths of the work. Typical criteria include: soundness of the claims (theoretical grounding, empirical evaluation), significance and novelty of the contribution, and relevance to the NeurIPS community.}\\
\noindent The paper gives a number of theoretical results for sequence-form optimization and a particular sequence-form regularizer. The authors do a good job of summarising the pieces of the proof, at a high level.\\

\noindent \textbf{3. Weaknesses: Explain the limitations of this work along the same axes as above.}\\
\noindent The paper might benefit from more clearly positioning its contributions. On one hand, it claims to sit in the domain of sequential decision making, using points from a sequence form representation rather than points in a simplex. On the other hand, by considering only the loss l.x the sequential decisions have effectively been collapsed, seemingly leaving this as a linear bandit problem with a slightly unusual convex action set.\\
    
\noindent \textbf{4. Correctness: Are the claims and method correct? Is the empirical methodology correct?}\\
\noindent I did not check the proofs, but the sketch is plausible and the bound is in line with other results.\\

\noindent Experiments:\\

\noindent  How many iterations did each algorithm use, in each experiment?\\

\noindent While it might only be applicable in the matrix game (and maybe Kuhn poker using normal form?), for a point of reference, how does something like EXP3 fare on the same plot?\\

\noindent The paragraph at line 110 states two differences from MCCFR, with the first being in bandit optimization, the strategy is output before the environment reveals feedback. This needs to be clarified: MCCFR seems to define a complete strategy at every iteration, before feedback is revealed. If this is not what is meant, what is meant?\\

\noindent The paragraph at line 320 states that in the experiments, 1) MCCFR was given the full information it requires, and 2) does not have a known guarantee of sublinear regret in this setting. Is claim 2 here that the fixed exploration used in online outcome sampling MCCFR adds a constant factor to the regret? If so, is this constant factor not handled by the standard doubling trick throughout bandit literature?\\

\noindent Further to the question about constant exploration, how was exploration handled in MCCFR in the experiments? The quality would seem to depend very much on the exploration constant, with the optimum choice depending on T.\\

\noindent Similarly, for AHR, the step size from Theorem 1 is based on T. How was T chosen, when the graph appears to be based on time?\\

\noindent There was manual parameter tuning used in these experiments: 5 times larger than the suggested theoretical value for the method in this paper and 2 times larger for AHR. What is the performance difference without this? Without this information, it's not clear whether one would expect to need to do some sort of parameter sweep to get reasonable performance.\\

\noindent What are the units displayed over time on the graphs? Regret / T? Normalised [0,1] units or natural game units?\\

\noindent \textbf{5. Clarity: Is the paper well written?}\\
\noindent The language in the paper is clear.\\
 
\noindent \textbf{6. Relation to prior work: Is it clearly discussed how this work differs from previous contributions?}\\
\noindent The paper discusses what seems to be a number of related works. However, as noted above, I think the paper could more clearly distinguish itself from other linear bandit work. I'm not sure I'm best positioned to offer the best choices for related work, but there seem to be closer matches than bandit convex optimisation or an algorithm for finding a game equilibrium.\\

\noindent As a possible concrete example, Section 1 refers to an $O(T^2/3)$ conjecture in "An optimal regret algorithm for bandit convex optimization". As per the paper cited there, "The special case of bandit linear optimization (BCO in case where the adversary is limited to using linear losses) is significantly simper [sic]." and cites a work on BLO. How does that work compare? Or, for another example, how does the work in this paper compare to bounds on sampled linear bandits in Theorem 28.10 in "Bandit Algorithms" (https://tor-lattimore.com/downloads/book/book.pdf\#page=342)\\

\noindent \textbf{7. Reproducibility: Are there enough details to reproduce the major results of this work?}\\
\noindent Yes\\

\noindent \textbf{8. Additional feedback, comments, suggestions for improvement and questions for the authors:}\\

\noindent In the introduction, line 50 mentions $O(\sqrt(T))$ for a prior algorithm, then uses $O(\sqrt(T \log T))$ in line 55. For minimum confusion, use the same statement in both places (or otherwise fix!)

\noindent  line 251 mentions an Algorithm 6 and line 292 mentions Lemma 11, both of which only appear within the appendix. The main body of the text should be a self-sufficient story: consider removing the reference as unnecessary, or if necessary, note they're part of a discussion in the appendix.\\

\noindent  -- comments after Author response\\

\noindent Thank you for the answers to the questions about the experiments. In my opinion, working those same clarifications into the experimental section would improve that section.\\

\noindent Some other thoughts:

\noindent - if it weren't for the good results, I might suggest removing most/all references to MCCFR, gven that it does not technically work in the setting. It requires a fair amount of explanation, and maybe adds some confusion given the number of MCCFR-related comments.

\noindent - I'm not sure what MCCFR with no exploration is. Even in the full-information case where it was developed, outcome sampling MCCFR requires an exploration policy at the agent's actions. Do the experiments just use the current policy? That would potentially be biased even in the full-information case.

\noindent - the results might have looked much different (MCCFR no longer works?) in an adversarial setting rather than a stochastic setting.\\
        
\noindent \textbf{9. Please provide an "overall score" for this submission.}\\
\noindent 4: An okay submission, but not good enough; a reject.\\

\noindent \textbf{10. Please provide a "confidence score" for your assessment of this submission.}\\
\noindent 4: You are confident in your assessment, but not absolutely certain. It is unlikely, but not impossible, that you did not understand some parts of the submission or that you are unfamiliar with some pieces of related work.\\

\noindent \textbf{11. Have the authors adequately addressed the broader impact of their work, including potential negative ethical and societal implications of their work?}\\
\noindent Yes\\


% Reviewer 2
% --------------------------------------------------------------------------------------

\subsection{Reviewer \#2}

\noindent \textbf{1. Summary and contributions: Briefly summarize the paper and its contributions.}\\
\noindent In this paper, the authors propose a new algorithm AHR for bandit linear optimization for sequential decision making (SDM). The regret bound of the the algorithm is proved to be $O(T)$ and the complexity in each iteration is linear time in the size of the decision tree.\\
    
\noindent \textbf{2. Strengths: Describe the strengths of the work. Typical criteria include: soundness of the claims (theoretical grounding, empirical evaluation), significance and novelty of the contribution, and relevance to the NeurIPS community.}\\
\noindent This paper presents a new regret minimization algorithm to solve extensive-form games without knowing counterfactual information. It's an interesting work.\\

\noindent \textbf{3. Weaknesses: Explain the limitations of this work along the same axes as above.}\\
\noindent (1) In general, the size of the decision tree grows exponentially and this is the main challenge in SDM. In the paper, numerical experiments only show some small examples and the algorithm does not show good performance on relatively large problem compared to MCCFR. Hence, I am very curious about the performance of the algorithm in large practical problems.\\

\noindent (2) The algorithm AHR looks like a general algorithm for bandit linear optimization. Does AHR take advantage of the structure of SDM and achieve better theoretical properties?\\

\noindent (3) What is the motivation of the definition of the weights $w_j$ in definition? Is the choice of the weights import for the proof?\\

\noindent (4) The MCCFR baseline is so weak, comparing with external sampling [1] and robust sampling [2] will be better.\\

\noindent [1] external sampling: https://papers.nips.cc/paper/3713-monte-carlo-sampling-for-regret-minimization-in-extensive-games.pdf\\

\noindent [2] robust sampling: https://openreview.net/pdf?id=ByedzkrKvH\\

\noindent \textbf{4. Correctness: Are the claims and method correct? Is the empirical methodology correct?}\\
\noindent (1) The authors claim they introduce a new regret minimization algorithm for SDM that does not use any counterfactual information. The define the counterfactual information as information on what would have happened had the agent chosen a different action at any decision point. However, some Monte Carlo CFR (MCCFR) variants, such as outcome sampling, external sampling and robust sampling, can also work without using any counterfactual information. For example, if the opponent takes action according to the current policy and player $i$ takes action according to her own current policy (outcome sampling) or uniform random policy (robust sampling), in MCCFR, the information set value can be computed without seeing the opponent's policy and actions.\\

\noindent (2) The experiment settings are so small. What's the performance on larger game?\\

\noindent (3) do you use exploration in MCCFR?\\

\noindent \textbf{5. Clarity: Is the paper well written?}\\
\noindent (1) The manuscript is in general well written and clear.\\

\noindent (2) The Algorithm 1 and Algorithm 2 are a little confusion. A full pseudo code would be better.\\

\noindent (3) The abstract is so long.\\

\noindent \textbf{6. Relation to prior work: Is it clearly discussed how this work differs from previous contributions?}\\
\noindent Yes.\\

\noindent \textbf{7. Reproducibility: Are there enough details to reproduce the major results of this work?}\\
\noindent Yes\\

\noindent \textbf{8. Additional feedback, comments, suggestions for improvement and questions for the authors:}\\
\noindent *Update after rebuttal*\\

\noindent The authors response to some of my confusions and I am not doubted about the new algorithm's improvements on regret bound and complexity in each iteration compared to the old algorithms AHR. The main concern is also whether MCCFR is well understood and properly compared. The setting of this paper is a little confusing and it is not very clear for me why MCCFR and many variants are not applicable for the setting. When using robust sampling, one player uses uniform random policy and the opponent uses its current strategy. This sampling schema is easy to be used in online problem. Hence, I trend to remain the mildly negative attitude, but I am willing to change my opinion if any reasonable clarification are provided.\\

\noindent \textbf{9. Please provide an "overall score" for this submission.}\\
\noindent 5: Marginally below the acceptance threshold.\\

\noindent \textbf{10. Please provide a "confidence score" for your assessment of this submission.}\\
\noindent 4: You are confident in your assessment, but not absolutely certain. It is unlikely, but not impossible, that you did not understand some parts of the submission or that you are unfamiliar with some pieces of related work.\\
    
\noindent \textbf{11. Have the authors adequately addressed the broader impact of their work, including potential negative ethical and societal implications of their work?}\\
\noindent Yes\\


% Reviewer 3
% --------------------------------------------------------------------------------------

\subsection{Reviewer \#3}

\noindent \textbf{1. Summary and contributions: Briefly summarize the paper and its contributions.}\\
\noindent This paper presents a bandit linear optimization algorithm tailored to sequential decision making problems, and its expected regret analysis. This method substantially outperforms a previous algorithm by Abernethy et al. (2008) and on small games it can even outperform outcome-sampled Monte-Carlo counterfactual regret minimization (CFR), which uses extra information about the realized action sequences on each round.\\

\noindent \textbf{2. Strengths: Describe the strengths of the work. Typical criteria include: soundness of the claims (theoretical grounding, empirical evaluation), significance and novelty of the contribution, and relevance to the NeurIPS community.}\\
\noindent This paper contributes a number of interesting theoretical observations and results. The new algorithm appears to be a substantial practical improvement over its predecessor, both in terms of its regret bound and its empirical performance in experiments.\\

\noindent A prime example is that the loss construction for the new algorithm sidesteps assumptions based on the minimum probability that any leaf is reached because even though this factor determines the conditioning of the autocorrelation matrix, and therefore also the norm of tilde{l}, the expected local dual norm is bounded by Theorem 2.\\

\noindent \textbf{3. Weaknesses: Explain the limitations of this work along the same axes as above.}\\
\noindent The motivation is muddled and weaker than it could be. This is the principle reason why my score for this paper is not higher.\\

\noindent The paper begins by describing sequential decision making (SDM) settings like Markov decision processes (MDPs), partially observable MDPs, and extensive-form games. Many common algorithms for these settings are based on experience samples, e.g., policy gradient or outcome sampling Monte-Carlo CFR, which require no counterfactual information (counter to the claim on lines 39-41). Allowing the learner access to the environment's execution information breaks the bandit assumption, but it is also a natural learning and execution model in these settings.\\

\noindent It is natural to ask players sequentially for actions as the game progresses according to the structure of the SDM process. Having each player instead declare their entire strategy upfront and have an external party sample an outcome according to the strategy profile appears substantially more artificial. Even ignoring the learning difficulties implied by the bandit execution model, which this paper seeks to address, the bandit execution model also imposes a significant computational burden on the players, who must each explicitly commit to an entire strategy on each round instead of individual decisions at only the realized information sets.\\

\noindent I could imagine that there are specialized settings where the bandit execution model is natural, maybe where the players and the environment are distributed in a way that players can more cheaply send one large message than many small messages about its actions at individual information sets, and it is cheaper for the environment to only send back utilities rather than the executed game history. There might also be privacy reasons why the game history should be hidden from each player. If applications like these were presented as motivation in place of general SDMs, the motivation would be much more clear and convincing. This critique extends to the choice of experimental settings as well.\\

\noindent \textbf{4. Correctness: Are the claims and method correct? Is the empirical methodology correct?}\\
\noindent I have not checked the details of the theoretical results, but the results themselves appear reasonable. I have a few questions about the experiments described in the "Additional feedback" section, but they also appear mostly reasonable and informative.\\

\noindent There are a couple of claims around MCCFR however that I find questionable:\\

\noindent 1. Lines 39-41 state that CFR methods require counterfactual information. Outcome sampling MCCFR estimates counterfactuals in a way that mimics the estimations done by Exp3 but on an information-set local basis. But the learner only receives reward information about actions that are actually part of its sampled experience. It is correct that this method relies on knowledge of the realized game information, which is unavailable in the bandit setting, but this is also less information than is provided in the semi-bandit setting. The semi-bandit setting gives learners access to rewards under different possible outcomes which are determined externally to the learner and is indeed counterfactual information wrt to any one of those outcomes\\

\noindent 2. In response to lines 119-120, MCCFR can be used to compute quantal-response equilibria by training MCCFR learners against quantal responses rather than than training them in self-play (Johanson et al., 2012; Davis et al., 2014) and it can be used to train safe exploitative strategies (Ponsen et al., 2011).\\

\noindent References\\
\noindent ==========\\
\noindent Johanson, Michael, et al. "Finding optimal abstract strategies in extensive-form games." Twenty-sixth AAAI conference on artificial intelligence. 2012.\\

\noindent Davis, Trevor, Neil Burch, and Michael Bowling. "Using response functions to measure strategy strength." Twenty-Eighth AAAI Conference on Artificial Intelligence. 2014.\\

\noindent Ponsen, Marc, Steven De Jong, and Marc Lanctot. "Computing approximate Nash equilibria and robust best-responses using sampling." Journal of Artificial Intelligence Research 42 (2011): 575-605.\\

\noindent \textbf{5. Clarity: Is the paper well written?}\\
\noindent This paper is clearly written and readable. Besides a few minor ambiguities around the experiments described in the "Additional feedback" section, I did not notice any clarity issues.\\
    
\noindent \textbf{6. Relation to prior work: Is it clearly discussed how this work differs from previous contributions?}\\
\noindent Except for questionable claims around MCCFR described in "Correctness", the prior work discussed appears complete and relevant.\\
    
\noindent \textbf{7. Reproducibility: Are there enough details to reproduce the major results of this work?}\\
\noindent Yes\\

\noindent \textbf{8. Additional feedback, comments, suggestions for improvement and questions for the authors:}\\
\noindent *Update after rebuttal*\\
\noindent Thanks for the rebuttal.\\

\noindent I was a little confused at first about running MCCFR without exploration, but I can see how the experiments ran, even though there is technically a problem with it and the regret bound is undefined. Where the strategy from regret matching is deterministic, the importance correction is just one, so it is a well defined estimate of the counterfactual value for the action taken at that information set. There is a 0/0 problem for the estimated counterfactual values at the unsampled actions but it is easy, if not technically correct, to just treat this as zero. This might be worth mentioning if the paper continues to include experiments with MCCFR.\\

\noindent I am happy that motivation specific to the bandit SDM problem will be added, but the statement that we should care about the bandit SDM problem simply because it is more restrictive is a little disappointing. As you have accepted, the interactive setting is more natural, algorithms for that setting can be much faster on large games (sampling actions on-demand rather than sampling one for each information set on each round), and they can make use of the information about which outcome actually ends up being sampled, so if we are giving up those nice properties we should get something in return. I am not sure that a compelling argument has been made for what has been gained beyond the value of generality for its own sake (which I agree is still worth something).\\

\noindent The fact that the lack of bandit SDM motivation and clarity around how this setting differs from the interactive setting where MCCFR sits led to some confusion in the other reviewers as well also caused me to weigh this aspect of the paper more highly.\\

\noindent Another reviewer pointed out that the experiments are performance against a fixed equilibrium component strategy, which I did not initially notice. I thought they showed regret during self-play, which would correspond to equilibrium approximation error. Performance against a fixed strategy is an extremely limited metric for evaluating regret minimizing algorithms. Even an unsound method (in terms of adversarial regret minimization) could perform very well on this task and accumulate low regret.\\

\noindent All of this has led me to reduce my score, though I still slightly favor acceptance due to the extensive theoretical work and computational benefits the new algorithm promises.\\

\noindent *Before rebuttal*
\noindent 1. The claim that ". . . if [the average regrets of the player converge to zero], the average strategies converge to a Nash equilibrium" on lines 67-69 is true of any algorithm, by the definition of average regret, so it is not specific to the new algorithm or Abernethy et al. (2008)'s, right? This statement could perhaps be clarified.\\

\noindent I also have some comments and questions about the experiments:\\

\noindent 2. The experimental results are presented in terms of regret, but is this the regret of the decisions that are actually made, or the strategies produced after each round? If it is the regret of the actual decisions, MCCFR's performance will be highly dependent on its uniform mixture parameter which is typically set very high (~0.6) since it is usually evaluated only on its final average strategy rather than its actual decisions. One way to avoid tuning this parameter would be to use Exp3 as the MCCFR learner instead of regret matching. Even if the regret is wrt the strategies themselves, this would also be a nice algorithm for comparison because it also reduces to Exp3 in matrix games. So MCCFR(Exp3) and the new algorithm then only diverge in games with decision sequences.\\

\noindent 3. In a matrix game, the new algorithm reduces to Exp3, but outcome sampling MCCFR also reduces to a bandit algorithm in this situation. The typical choice of the learner for MCCFR is regret matching, so this experiment is simply comparing Exp3 to outcome sampled regret matching, correct? The matrix game results is surprising to me because outcome sampled regret matching tends to perform at least as well as Exp3 with a well tuned temperature after the same number of rounds, but regret matching tends to be faster since it does not require exponentiation.\\

\noindent 4. Since all of the algorithms compared in experiments are iterative and iterations have roughly the same meaning for each, it might be instructive to show performance relative to the number of iterations, in addition to time. The reason why this might be useful is to provide a more thorough and favorable comparison with MCCFR. MCCFR is cheating compared to the new algorithm in two ways: its strategy is computed, sampled, and updated only at observed decision points and it is allowed to observe the decisions of the other players. So MCCFR updates can be done faster, and this advantage scales with the size of the game. But this unfair speed advantage is nullified if the algorithms are compared across iterations. While MCCFR still has the advantage of observing the actions of the other players, I expect the performance gaps in the larger games to close considerably within this framing.\\

\noindent 5. The Leduc game used in experiments has been reduced to its canonical form, correct? Otherwise 337 would be too few sequences. This might be worth clarifying.\\

\noindent \textbf{9. Please provide an "overall score" for this submission.}\\
\noindent 6: Marginally above the acceptance threshold.\\

\noindent \textbf{10. Please provide a "confidence score" for your assessment of this submission.}\\
\noindent 4: You are confident in your assessment, but not absolutely certain. It is unlikely, but not impossible, that you did not understand some parts of the submission or that you are unfamiliar with some pieces of related work.\\
    
\noindent \textbf{11. Have the authors adequately addressed the broader impact of their work, including potential negative ethical and societal implications of their work?}\\
\noindent Yes\\

% Reviewer 4
% --------------------------------------------------------------------------------------

\subsection{Reviewer \#4}

\noindent \textbf{1. Summary and contributions: Briefly summarize the paper and its contributions.}\\
\noindent The paper proposes an online optimisation algorithm for sequential decision making in the bandit setting (i.e. no counterfactual information) assuming a linear loss (linear w.r.t. the decisions). The authors claim to provide the first bandit optimization algorithm for SDM. Moreover it improves on existing bandit regret minimizers (defined more generally for convex sets) both in terms of performance (regret bounds) and computational complexity.\\

\noindent The algorithm “estimates” counterfactual estimation from the scalar loss. It then uses this artificial signal to minimize regret using mirror descent. It also uses a regularizer called “dilated entropy distance-generating function” which brings two advantages: (1) efficient optimisation that reduces to linear traversals of the decision path; (2) it defines a norm which leads to a tight bound for the expected regret.\\

\noindent The paper consists of solid theoretical work, having proofs for the bounds mentioned above.\\

\noindent \textbf{2. Strengths: Describe the strengths of the work. Typical criteria include: soundness of the claims (theoretical grounding, empirical evaluation), significance and novelty of the contribution, and relevance to the NeurIPS community.}\\
\noindent- Clearly stated claims that have theoretical support.\\
\noindent- Fair empirical validation that show good performance.\\
\noindent- Originality: bridges bandit approaches for one-shot decision problems with sequential decision making where previous learning algorithms used counterfactual information to minimise risk. (authors claim this is only the second work to *efficiently* address this combination: bandit + sequential decisions; and the first one [1] addressed convex sets in general)\\
\noindent- Good complexity for the expected cumulative regret (O(sqrt(T)) and linear-time per iteration.\\
\noindent- Several interesting theoretical results on the side.\\

\noindent \textbf{3. Weaknesses: Explain the limitations of this work along the same axes as above.}\\
\noindent The main limitation of the current work is the result that bounds the regret in expectation, meaning that for certain cases regret might be arbitrarily large. The authors also state this in the paper several times.\\

\noindent \textbf{4. Correctness: Are the claims and method correct? Is the empirical methodology correct?}\\
\noindent Statements have detailed proofs. Experiments seem to demonstrate the performance gain of the current algorithm.\\

\noindent I appreciate the fact that the authors are honest about the limitations of their approach (e.g. they stress the difference between bounding the maximum value for the regret and bounding its expectation).\\

\noindent \textbf{5. Clarity: Is the paper well written?}\\
\noindent There are a few details that are exclusively in the Appendix, and that would need some explaining in the paper. E.g. explaining the importance of the upper bound in theorem 1 and introducing eta.\\

\noindent Also, paragraph 227-231 talks about the use of the autocorrelation matrix to deal with exploration, but this is not discussed in any way. Exploration is an interesting aspect of the problem, so it would be better to have a paragraph actually discussing it.\\

\noindent \textbf{6. Relation to prior work: Is it clearly discussed how this work differs from previous contributions?}\\
\noindent I am not familiar with the field, but I got a good understanding of the landscape of the existing approaches from this article. Also, the paper addresses the differences between their work and Abernethy et al. [1], the only other study that has results comparable to the current one. I.e. the cost per iteration was cubic in [1], while here is linear. Also, current paper's bound is tighter.\\
    
\noindent \textbf{7. Reproducibility: Are there enough details to reproduce the major results of this work?}\\
\noindent Yes\\
    
\noindent \textbf{8. Additional feedback, comments, suggestions for improvement and questions for the authors:}\\
\noindent8: Top 50\% of accepted NeurIPS papers. A very good submission; a clear accept.\\
    
\noindent \textbf{9. Please provide an "overall score" for this submission.}\\

\noindent \textbf{10. Please provide a "confidence score" for your assessment of this submission.}\\
\noindent 3: You are fairly confident in your assessment. It is possible that you did not understand some parts of the submission or that you are unfamiliar with some pieces of related work. Math/other details were not carefully checked.\\
    
\noindent \textbf{11. Have the authors adequately addressed the broader impact of their work, including potential negative ethical and societal implications of their work?}\\
\noindent Yes\\

% Meta-Reviewer 1
% --------------------------------------------------------------------------------------

\subsection{Meta-Reviewer \#1}

\noindent \textbf{1. Please recommend a decision for this submission.}\\
\noindent Reject\\

\noindent \textbf{3. Please provide a meta-review for this submission. Your meta-review should explain your decision to the authors. It should augment the reviews and communicate how the reviews, author response, and discussion were used to arrive at a decision. Dismissing or ignoring a review is not acceptable unless you have a good reason for doing so. If you want to make a decision that is not clearly supported by the reviews, perhaps because the reviewers did not come to a consensus, please justify your decision appropriately, including, but not limited to, reading the submission in full and writing a detailed meta-review that explains your decision.}\\
\noindent The paper describes a method for sequential decision-making based on bandit linear optimization in order to employ regret minimization without the requirement of exploration. A regret bound is obtained for this setting.\\

\noindent The reviews agreed that the problem is interesting and worthy of investigation, but the motivation is largely occluded by a convoluted positioning related to previous work. Three of the four reviewers who understood the paper brought this point up, and it was the most discussed point in the discussion. The reviewers were unable to consolidate an understanding for this line of motivation. My first reaction based on looking at page 3 is precisely the same as Reviewer 3's: the fact that the bandit algorithm has to decide the entire strategy up front is a restrictive assumption, it is not clear that this is more practical than being able to sample interactively with forced exploration. As Reviewer 1 points out, this point is belabored and the space could be better used; perhaps the requirement of sampling up front would be less problematic if the empirical results showed that in addition to the regret bound that the approach leads to better results in self-play, or against adaptive/switching opponents, or against known sub-optimal opponents. In any case, this motivation requires some further thought.\\

\noindent In addition, a point about the results being against a fixed adversary rather than is self-play was brought up and discussed, altering the opinion of one reviewer.\\

\noindent The discussion also brought up a number of follow-up question from Reviewer 3. I encourage the authors to take all of this feedback into account when revising the paper.\\


